Probe position determination with multichannel I-V measurements in a two-dimensional sheet$\colon$ Computational method and mathematical analysis

Atomically thin films and surfaces exhibit many distinctive two-dimensional electronic properties that are absent in bulk crystals. In situ microscale multi-probe measurements have been utilized as an effective method to identify the electrical conductivity of such thin films and surfaces. Precise determination of multi-probe positions is crucial for accurate characterization of the conductance. However, traditional methods that use microscopes for determining multi-probe positions often impose significant constraints on experimental setups. In some cases, installing a microscope is not even feasible. Therefore, in this study, we propose a novel method to determine probe positions using electrical signals from the probes. This method enables precise determination of probe positions using a reference sheet and reference probes, even at low or high temperatures and under ultra-high vacuum or high-pressure conditions. The proposed method simplifies the integration of microscale multi-probe measurement systems into various devices, thereby advancing research on thin films and surfaces.

==> latexmkrc <==
#!/usr/bin/perl

# How to Use ############################################################ 
# 
# For Japanese articles:
#       * Uncomment "Use platex" and comment out "Use pdflatex" in 1.
#       * Uncomment 3.
#       * Set 4. to "3"
#
# For English articles:
#       * Uncomment "Use pdflatex" and comment out "Use platex" in 1.
#       * Comment out 3.
#       * Set 4. to "1"
# 
#########################################################################

#--------------------------------------------------#
# 1. Compile Command Setting
#--------------------------------------------------#

##### Use platex (for Japanese articles) #####
$latex = 'uplatex %O -src-specials -shell-escape -file-line-error -halt-on-error -interaction=nonstopmode -synctex=1 -kanji=utf8 %S';

##### Use pdflatex (for English articles) #####
# $latex = 'pdflatex %O -src-specials -file-line-error -halt-on-error -interaction=nonstopmode -synctex=1 -kanji=utf8 %S';

#--------------------------------------------------#
# 2. BibTeX Setting (if you use bibtex to make references)
#--------------------------------------------------#

$bibtex = 'pbibtex %O %B -kanji=utf8';

#--------------------------------------------------#
# 3. DVI-PDF Converter Setting (if you make pdf from dvi)
#--------------------------------------------------#

$dvipdf = 'dvipdfmx %O -o %D %S';

#--------------------------------------------------#
# 4. PDF Mode Setting
#   0: don't make pdf
#   1: use pdflatex (English)
#   2: use ps2pdf
#   3: make pdf from dvi (Japanese)
#--------------------------------------------------#

$pdf_mode = 3; 

#--------------------------------------------------#
# 5. Previewer Settings
#--------------------------------------------------#

##### Use pdf-view of tex editors #####
$pdf_previewer = 'exit';

##### If you use external previewers (you have to verify paths of pdf previewers and tex editors) #####
##### Use SumatraPDF and VS code inverse search #####
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\Programs\Microsoft VS Code\Code.exe\" -g \"%f\":\"%l\"" %O %S';

##### Use SumatraPDF and Atom inverse search #####
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

#--------------------------------------------------#
# 6. Other Settings
#--------------------------------------------------#

##### Don't preserve temporary files #####
# $pvc_view_file_via_temporary = 0;

#--------------------------------------------------#
# References
# * https://ichiro-maruta.blogspot.com/2016/01/atom-latex-on-windows.html
# * https://qiita.com/Rumisbern/items/d9de41823aa46d5f05a8
#--------------------------------------------------#

